SudokuSens: Enhancing Deep Learning Robustness for IoT Sensing Applications using a Generative Approach

This paper introduces SudokuSens, a generative framework for automated generation of training data in machine-learning-based Internet-of-Things (IoT) applications, such that the generated synthetic data mimic experimental configurations not encountered during actual sensor data collection. The framework improves the robustness of resulting deep learning models, and is intended for IoT applications where data collection is expensive. The work is motivated by the fact that IoT time-series data entangle the signatures of observed objects with the confounding intrinsic properties of the surrounding environment and the dynamic environmental disturbances experienced. To incorporate sufficient diversity into the IoT training data, one therefore needs to consider a combinatorial explosion of training cases that are multiplicative in the number of objects considered and the possible environmental conditions in which such objects may be encountered. Our framework substantially reduces these multiplicative training needs. To decouple object signatures from environmental conditions, we employ a Conditional Variational Autoencoder (CVAE) that allows us to reduce data collection needs from multiplicative to (nearly) linear, while synthetically generating (data for) the missing conditions. To obtain robustness with respect to dynamic disturbances, a session-aware temporal contrastive learning approach is taken. Integrating the aforementioned two approaches, SudokuSens significantly improves the robustness of deep learning for IoT applications. We explore the degree to which SudokuSens benefits downstream inference tasks in different data sets and discuss conditions under which the approach is particularly effective.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> content/cut-figure.tex <==
\begin{figure*}[htbp]
    \centering
    % First row of images
        \centering
        \begin{subfigure}[b]{0.139\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figure/scenarios/scenarioA.jpg}
            \caption{}
            \label{fig:scenarioA}
        \end{subfigure}
        \begin{subfigure}[b]{0.139\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figure/scenarios/scenarioB.jpg}
            \caption{}
            \label{fig:scenarioB}
        \end{subfigure}
        \begin{subfigure}[b]{0.139\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figure/scenarios/scenarioC.jpeg}
            \caption{}
            \label{fig:scenarioC}
        \end{subfigure}
        \begin{subfigure}[b]{0.139\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figure/scenarios/scenarioD.jpeg}
            \caption{}
            \label{fig:scenarioD}
        \end{subfigure}
        \begin{subfigure}[b]{0.139\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figure/scenarios/scenarioE.jpeg}
            \caption{}
            \label{fig:scenarioE}
        \end{subfigure}
        \begin{subfigure}[b]{0.139\textwidth}
            \centering
            \includegraphics[width=\linewidth]{figure/scenarios/scenarioF.jpeg}
            \caption{}
            \label{fig:scenarioF}
        \end{subfigure}
        \begin{subfigure}[b]{0.139\textwidth}
            \centering
            \includegraphics[width=\textwidth]{figure/scenarios/scenarioG.jpeg}
            \caption{}
            \label{fig:scenarioG}
        \end{subfigure}

        \caption{Scenarios of collecting data. Each scenario is a unique combination of location and environmental factors.}
        \label{fig:scenarios}
\end{figure*}

==> content/discussion.tex <==
\section{Discussion}
\label{sec:discussion_and_future_work}

% How to decide intrinsic attributes and dynamic disturbances
SudokuSens offers a general framework for enhancing the robustness of deep learning models in IoT sensing. Yet, its customization for specific IoT applications requires identifying influential factors as intrinsic attributes or dynamic disturbances.
SudokuSens, as its name implies, can only interpolate unseen conditions if their attributes have already appeared in known conditions. This is due to the one-hot embedding of each attribute value in the conditional vector during conditional interpolation.  
One concern regarding SA-TCL is how to avoid dimensional collapse, which refers to the situation where all data samples, regardless of their labels or content, are mapped to the same or very similar points in the embedding space\cite{jing2021understanding}. In our current implementation, we rely on manually setting the proper learning rate and training epoch to fine-tune SA-TCL to the optimal performance. However, it would be good to propose a smarter positive pairs construction algorithm, like considering both the local and global temporal relationships used in video temporal contrastive learning\cite{dave2022tclr}.

% future work

==> content/old-discussion.tex <==
\section{Discussion}
\label{sec:discussion_and_future_work}

% How to decide intrinsic attributes and dynamic disturbances
SudokuSens offers a general framework for enhancing the robustness of deep learning models in IoT sensing. Yet, its customization for specific IoT applications requires identifying influential factors as intrinsic attributes or dynamic disturbances.
\textcolor{blue}{In practice, intrinsic attributes are factors that impose a constant influence on the sensing signals. 
These factors are usually closely bound to the sensing target itself (like the physical structure or the texture of the surface), or environmental variables that pose a stable impact on the transmission of the signal to the sensor (such as the transmission media).
Easily labeled during data collection, these attributes are used for synthesizing new samples through conditional interpolation. 
In contrast, dynamic disturbances, which are hard to label, represent temporal state variations and often stem from stochastic environmental noises or different observations of the same physical phenomenon}
\textcolor{blue}{In vehicle detection application, the vehicle type is taken as an intrinsic attribute as it determines the physical structure of the target object, which remains constant.}
Terrain at the location is also regarded as an intrinsic attribute. This assumption was based on the fact that the fields where we collected data were mostly flat, providing a relatively static medium for transmitting vibration and generating sound. However, if the field is irregular and uneven, this assumption no longer holds. In such cases, it might be necessary to take terrain as a dynamic disturbance and address it during SA-TCL. 
\textcolor{blue}{Environmental noises in vehicle detection were addressed as dynamic disturbances and handled by SA-TCL.
This is based on the fact that during the data collection, the traffic noises and wind noises are temporally changing instead of an ideal constant Gaussian noise.
Similarly, the speed and the distance to sensor also temporally influence the received signals.
They are hard to label and unrelated to the classification task.}
\textcolor{blue}{In HAR applications, human subjects are classified as the intrinsic attribute. 
The logic behind is that the identity of the human subject summarizes the physiological metrics of the target, such as weight, height, strength, and movement pattern. 
Those are stable influential factors to the sensing signals and they are easy to be labeled.
Meanwhile, the variances that exist in their different attempts of the same activity are taken as dynamic disturbances.
The variances come from the different movement intensities and speeds, which may significantly impact the sensing signals.}
\textcolor{blue}{
Given the discussion above, a major limitation of SudokuSens is that the feature design decisions have to be made by the users based on their pre-knowledge and understanding of the specific IoT sensing application.}

% Seen attributes only, 
SudokuSens, as its name implies, can only interpolate unseen conditions if their attributes have already appeared in known conditions. This is due to the one-hot embedding of each attribute value in the conditional vector during conditional interpolation.  
\textcolor{blue}{A more ideal solution for handling unseen attributes could be empowering SudokuSens the ability of extrapolation.
Given various values of the same attribute (like types of the vehicle), SudokuSens needs to learn the relationships/distances among them, and predict the influence comes from a new value.
To realize that, we require finer-grained data labeling (like the weights, engine parameters, wheel sizes of the vehicles), which again puts a heavy burden on the dataset development.}
Another possible solution could be using a language model to encode detailed scenario descriptions or keywords into a conditional vector\cite{li2020sentence, huang2021disentangling}. This could enrich conditions and enhance sample diversity via the CVAE, allowing SudokuSens to {\em extrapolate\/} conditions. However, it introduces challenges, such as ensuring quality textual descriptions, collecting appropriate training data, and handling interpretability.

% Review #24C: Section 4.4, in this part, it was confirmed that when there is no gap, performance may be lower than that of the existing baseline. Gaps will change frequently in the real environment, so what strategies can be taken to flexibly prepare for such cases when using SudokuSense?
\textcolor{blue}{As stated in Section~\ref{subsec:overall_performance}, SudokuSens sometimes exhibits negative influence when there is no gap between the development scenarios and the deployment scenarios.
We speculate that it is because the synthetic samples have lower quality in the sense of representing the real-world physics, and potentially introduce errors in recombining the influences from the intrinsic attributes. 
When there is no realistic samples under a condition, the synthetic samples positively act as reasonable suggestions to the downstream model about the potential signal transformation.
However, when sufficient realistic samples exist, the synthetic samples might dilute the overall quality of the training dataset, potentially leading to a negative influence.
Given that limitation, users of SudokuSens need to balance between the benefits brought to the out-dataset conditions, and the potential "quality dilution effect" on the in-dataset conditions.
Despite of that, based on our experiments, SudokuSens still brings slight performance improvement in most cases when there is not gap, showing a low risk of sabotaging the overall performance. 
}

% Constrained by labeled datasets
One concern regarding SA-TCL is how to avoid dimensional collapse, which refers to the situation where all data samples, regardless of their labels or content, are mapped to the same or very similar points in the embedding space\cite{jing2021understanding}. In our current implementation, we rely on manually setting the proper learning rate and training epoch to fine-tune SA-TCL to the optimal performance. However, it would be good to propose a smarter positive pairs construction algorithm, like considering both the local and global temporal relationships used in video temporal contrastive learning\cite{dave2022tclr}.

% future work

==> content/stale_content/introduction_old.tex <==
\section{introduction}

% Meaning of contrastive learning:
% if the labeled data is relatively small or if the input features are complex and high-dimensional, contrastive learning can be used to pre-train a deep neural network to learn a good representation of the input data. This pre-trained network can then be fine-tuned for the specific supervised learning task, which can lead to improved performance and better generalization.

In contrast to research fields such as natural language processing, computer vision, and social media, datasets in the realm of sensor-based human activity recogniton (HAR) are frequently limited in scale. Previous research in HAR has often collected data in experimental environments that are not sufficiently comprehensive to cover real-world scenarios. Experience has shown that training deep learning models on limited datasets can result in catastrophic failures during deployment due to overfitting. Therefore, a critical question arises: How can we mitigate the overfitting of deep learning models when we only have access to a limited amount of data in HAR?

Overfitting occurs when deep learning models capture noise or random variations instead of the true underlying relationships in the data. To mitigate overfitting under the constraints of limited datasets, one approach is to guide the neural network to learn more fundamental features. Previous research has shown promising results using feature extraction to combat overfitting. However, fundamental feature extractions usually rely on big data\cite{foundation_model}, or symbolic reasoning \cite{neuro_symbolic} as guidance. In HAR, however, big data is not always available, while symbolic reasoning like depicting the underlying physical rules of the human movements is too complicated.  While it may be difficult to directly guide the neural network to learn fundamental features, we can explicitly guide it to avoid learning activity-irrelevant variations. We argue that one external knowledge can be leveraged to overcome overfitting comes from the sources of activity-irrelevant variations. We categorize the sources of into two categories: the time-variant states and the time-invariant attributes. Time-variant states refer to the dynamic aspects of human activities that change over time, such as the speed, duration, and intensity of an activity. These temporal states are challenging to label because the intensity and speed of a physical activity can vary greatly through time. On the bright side, incorporating diversity of states into the dataset is inexpensive, as during data collection, the human objects naturally perform the same activity in different intensities, speeds or durations. In contrast, time-invariant attributes are easier to label, as we can clearly identify the human object and environment. We can easily label all the samples under the same session of data collection by an attribute set, such as "personA-room1", "personB-room2". But it is harder to collect diverse data samples for attributes. This is because they are intrinsic to the human object and the environments, and therefore require more resources to collect data samples from different human objects and environments to capture the full range of variations. 

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth,trim={0.1cm 0 0 5.8cm},clip]{figure/framework.pdf}
\caption{RobustHAR}
\label{fig:framework}
\end{figure}


Based on the above insights, we propose a data augmentation framework called RobustHAR for handling the two sources of unrelated variations that may confound the deep learning models in HAR. For time-variant states, we utilize a temporal contrastive learning neural network to mitigate the variance that arises from different time steps. An important insight that informs this approach is that HAR datasets are typically organized into multiple sessions of data collection. Specifically, HAR datasets are usually collected by asking a human object to perform a certain activity for a duration of time. This process is repeated on different activities by different human objects and probably in different environments to obtain a complete dataset. Within each session, the data samples are temporally continuous and pertain to the same activity class. We propose a multimodal convolutional neural network for temporal contrastive learning, which takes the short-time Fourier transformed spectrograms from the original time-series data as input. The contrastive learning network treats the signal samples from the same run as positive pairs and those from different runs as negative pairs. By encouraging the samples within the same run to be closer in the latent space and pushing the samples from different runs farther apart, the contrastive learning encoder is able to learn to mitigate the temporal variance while preserving the time-invariant activity-related features. The trained encoder will further be used as the first stage of RobustHAR pipeline during data augmentation.


For time-invariant factors, RobustHAR uses a conditional variational autoencoder (cVAE) to augment the dataset. As we mentioned earlier, it is usually more expensive to incorporate the diversity in time-invariant attributes, such as human objects and environments. Hence, it is a common case that in a realistic HAR application, we only have training data under partially sampled conditions. These conditions may include different human objects with varying physical characteristics, as well as different environmental settings. Due to practical limitations, it may not be possible to collect data for all possible combinations of these conditions. As a result, the training dataset may only contain a subset of these conditions. This can make it difficult for a deep learning model to generalize to unseen conditions and lead to overfitting or poor performance. To handle this, we uses a conditional variational autoencoder (cVAE) which takes the time-invariant attributes as additional information for modeling the inputs. After training the cVAE on the training dataset, we input the interpolated missing conditions in the original dataset to the cVAE decoder to generate non-existing samples. This augmentation process results in a complete conditional sampling dataset that help mitigate the bias of the downstream HAR model towards the conditions present in the original dataset. The augmented dataset will be taken as the input for the downstream HAR classifier.

In general, we summarize our contributions as follows:

\begin{enumerate}
    \item We propose a data augmentation framework called RobustHAR for improving the robustness of the HAR models under data scarcity. RobustHAR does not rely on any general big dataset or symbolic embedding of the physics, which makes it practical enough to be applied to many HAR applications with small-scale datasets.
    \item In RobustHAR, we innovatively leverage the external knowledge about what are \textbf{irrelevant} to the human activities to guide the downstream model to learn more fundamental features. Following this intuition, we further categorize the sources of causing the activity-irrelevant variations in the sensor signals into two sources, and address them separately.
    \item For the first source of activity-irrelevant variations: time-variant states, we adopt temporal contrastive learning to mitigate the time-variant noises. We also propose an optimization for contrastive learning on short-time Fourier transformed spectrograms.
    \item For time-invariant attributes, we employ a conditional variational autoencoder to complement the missing conditions in the original dataset. Conditional interpolation approach helps to ensure that the downstream model is able to accurately generalize to new conditions that were not present in the original dataset.
    \item We conduct comprehensive experiments to show that your framework greatly improves the robustness of deep learning models in HAR on unseen conditions. We perform ablation studies to validate the effectiveness of each component in RobustHAR.
\end{enumerate}



% \begin{figure*}[h!]
% \centering
% \includegraphics[width=1\linewidth]{figure/robustiot.pdf}
% \caption{RobustIoT}
% \label{fig:robust_iot}
% \end{figure*}



% \begin{figure*}[h!]
% \centering
% \includegraphics[width=\linewidth,trim={0.1cm 0 0 3.3cm},clip]{figure/tempclr.pdf}
% \caption{Temporal Contrastive Learning}
% \label{fig:tempclr}
% \end{figure*}

% By incorporating both time-variant and time-invariant factors into our framework, we aim to improve the robustness of deep learning models in IoT applications, particularly in scenarios where limited labeled data is available.



% \begin{figure}[h!]
% \centering
% \includegraphics[width=1\linewidth]{figure/condition_interp.pdf}
% \caption{Condition interpolation: a vehicle type recognition example}
% \label{fig:condition_interp}
% \end{figure}


% Based on this observation, RobustIoT handles each type of influential factors separately. For time-variant factors, RobustIoT uses a temporal contrastive learning neural network to reduce the variance brought in different time steps. One insight is that the IoT dataset is usually organized in multiple runs of data collection. Take motion-sensor-based vehicle type recognition task as an example, we collect data by running a vehivlce on a terrain at different speeds and distances for a certain time. We repeat this process on different vehicle-terrain combinations, and get the complete dataset. Within each run, the data points are temporally continuous and belong to the same vehicle type. The contrastive learning network takes the signal samples from the same run as positive pairs, and samples from different run as negative pairs. By pulling the samples within the same run closer in the latent space while pushing the samples from different runs farther, the contrastive learning encoder learns to ignore the temporal variance while keep the time-invariant features. 


% Building on this observation, RobustIoT employs a strategy of handling each type of influential factor separately. To address time-variant factors, RobustIoT utilizes a temporal contrastive learning neural network to mitigate the variance that arises from different time steps. An important insight that informs this approach is that IoT datasets are typically organized into multiple runs of data collection. For example, in a motion-sensor-based vehicle type recognition task, data is collected by running a vehicle on a terrain at different speeds and distances for a specified duration of time. This process is repeated on different vehicle-terrain combinations to obtain a complete dataset. Within each run, the data points are temporally continuous and pertain to the same vehicle type. The contrastive learning network treats the signal samples from the same run as positive pairs and those from different runs as negative pairs. By encouraging the samples within the same run to be closer in the latent space and pushing the samples from different runs farther apart, the contrastive learning encoder is able to learn to ignore the temporal variance while preserving the time-invariant features. 


% They are naturally the multi views of the same phenomenon!

% For time-invariant factors, RobustIoT uses a conditional variational autoencoder (cVAE) to augment the dataset. As we mentioned earlier, it is usually more expensive to incorporate the variance caused by time-invariant factors. Hence, it is a common case that in IoT datasets, we only have partially sampled conditions. The cVAE takes the time-invariant labels as additional information for modeling the inputs. After training the cVAE on the training dataset, we input the interpolated missing conditions in the original dataset to the cVAE decoder to generate non-existing samples. 



% \begin{table*}[]
% \caption{Influential Factors in Typical IoT Applications}
% \label{tab:iot_app_comparision}
% \centering

% \begin{tabular}{|l|l|l|l|}
% \hline
% & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Human Activity\\ Recognition\end{tabular}}}   & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Vehicle Type \\ Recognition\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Earthquake \\ Detection\end{tabular}}} \\ \hline \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}Time-variant factors\end{tabular}}   & \begin{tabular}[c]{@{}l@{}}Activity speed, \\ Activity intensity, Distance to sensors\end{tabular} & \begin{tabular}[c]{@{}l@{}}Vehicle speed,\\ Distance to sensors\end{tabular} & Wave speed \\ \hline
% \textbf{\begin{tabular}[c]{@{}l@{}}Time-invariant factors\end{tabular}} & Environment, & Terrain type & Terrain type \\ \hline
% \textbf{Sensing target} & Human activity type & Vehicle type  & \begin{tabular}[c]{@{}l@{}}Earthquake or not
% \end{tabular} \\ \hline
% \end{tabular}
% \end{table*}


==> content/tables/dataset_performance.tex <==
\begin{table*}[ht]
\centering
\resizebox{0.3\textwidth}{!}{\input{content/tables/dataset_performance_acids}}
\quad
\resizebox{0.3\textwidth}{!}{\input{content/tables/dataset_performance_wear-har}}
\quad
\resizebox{0.3\textwidth}{!}{\input{content/tables/dataset_performance_wifi-har}}
\caption{Your caption goes here.}
\label{tab:my_label}
\end{table*}

==> content/tables/dataset_performance_acids.tex <==
\begin{tabular}{|l|l|llllll|}
\hline
\multirow{3}{*}{Method} & \multirow{3}{*}{Classifier} & \multicolumn{6}{l|}{Gap}                                                                                                                \\ \cline{3-8} 
                        &                             & \multicolumn{2}{l|}{2}                             & \multicolumn{2}{l|}{1}                             & \multicolumn{2}{l|}{0}        \\ \cline{3-8} 
                        &                             & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{Acc} & F1 \\ \hline
Basic                   & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
Augmented               & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
TNC                     & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
TF-C                    & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
SudokuSens              & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
\end{tabular}


==> content/tables/dataset_performance_wear-har.tex <==
\begin{tabular}{|l|l|llllll|}
\hline
\multirow{3}{*}{Method} & \multirow{3}{*}{Classifier} & \multicolumn{6}{l|}{Gap}                                                                                                                \\ \cline{3-8} 
                        &                             & \multicolumn{2}{l|}{2}                             & \multicolumn{2}{l|}{1}                             & \multicolumn{2}{l|}{0}        \\ \cline{3-8} 
                        &                             & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{Acc} & F1 \\ \hline
Basic                   & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
Augmented               & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
TNC                     & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
TF-C                    & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
SudokuSens              & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
\end{tabular}


==> content/tables/dataset_performance_wifi-har.tex <==
\begin{tabular}{|l|l|llllll|}
\hline
\multirow{3}{*}{Method} & \multirow{3}{*}{Classifier} & \multicolumn{6}{l|}{Gap}                                                                                                                \\ \cline{3-8} 
                        &                             & \multicolumn{2}{l|}{2}                             & \multicolumn{2}{l|}{1}                             & \multicolumn{2}{l|}{0}        \\ \cline{3-8} 
                        &                             & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{Acc} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{Acc} & F1 \\ \hline
Basic                   & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
Augmented               & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
TNC                     & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
TF-C                    & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
SudokuSens              & Shalow                      & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & DeepSense                   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
                        & Transformer                 & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    & \multicolumn{1}{l|}{}   & \multicolumn{1}{l|}{}    &    \\ \hline
\end{tabular}

